Progressively-connected Light Field Network for Efficient View Synthesis

This paper presents a Progressively-connected Light Field network (ProLiF), for the novel view synthesis of complex forward-facing scenes. ProLiF encodes a 4D light field, which allows rendering a large batch of rays in one training step for image- or patch-level losses. Directly learning a neural light field from images has difficulty in rendering multi-view consistent images due to its unawareness of the underlying 3D geometry. To address this problem, we propose a progressive training scheme and regularization losses to infer the underlying geometry during training, both of which enforce the multi-view consistency and thus greatly improves the rendering quality. Experiments demonstrate that our method is able to achieve significantly better rendering quality than the vanilla neural light fields and comparable results to NeRF-like rendering methods on the challenging LLFF dataset and Shiny Object dataset. Moreover, we demonstrate better compatibility with LPIPS loss to achieve robustness to varying light conditions and CLIP loss to control the rendering style of the scene. Project page: https://totoro97.github.io/projects/prolif.

==> 1_intro_bak.tex <==
\section{Introduction}
% key idea: large training batch size 
% 1. nerf quality is high but training batch size is small. training nerf mainly rely on RGB loss on single ray. large training batch size is usefule and an intriguing property for some applications. 
% 3. light field based methods can use large training batch size but have difficulty in handling consistency. 
% 4. we propose a new representation keep consistency
% 5. fast rendering with small memory footprint.
% 6. experiments.
Rendering free-viewpoint photo-realistic images from camera captures is a long-standing problem in computer vision, multimedia and graphics. This task, which we usually call image based rendering (IBR) or novel view synthesis (NVS), has many practical applications such as gaming, augmented reality, human-computer interaction, etc. % Given a set of posed images as inputs, the goal of IBR is to render novel images from arbitrary poses.

% ----- Drawbacks of NeRF -----
In recent years, the image quality of IBR has been improved dramatically with the recent fashions of Neural Radiance Fields (NeRF)~\cite{mildenhall2020nerf}. The basic idea of NeRF is representing the scene as a 5D radiance field as well as a 3D spatial volume density field, encoded by the Multi-layer Perceptrons (MLPs). To render a pixel color of an image, NeRF first samples a sequence of points along the corresponding emit ray, and query the colors and volume densities of these point samples. Then the color is synthesized by the classic volume rendering technique on top of the queried colors and densities. This rendering process is differentiable, therefore NeRF can be optimized and can learn a compact neural scene representation that fits the image captures. Though NeRF achieves photo-realistic results of novel views, the inferring speed of it is rather slow. For example, rendering an image with ~1M pixels typically costs around a minute. This issue is mainly due to that NeRF needs hundreds of point samplings (as well as the number of network evaluations) for volume rendering to synthesize the color of only one single pixel.

% NeRF - Speed up with data structure
More recently, some works have successfully addressed the slow rendering problem of NeRF by introducing hybrid representations (i.e., the combination of neural networks and explicit data structures)~\cite{liu2020neural,yu2021plenoctrees,reiser2021kilonerf,hedman2021baking,garbin2021fastnerf} to reduce the number of point samplings. Moreover, some of them have even achieved real-time rendering in the inference stage~\cite{yu2021plenoctrees,reiser2021kilonerf,hedman2021baking,garbin2021fastnerf}. However, they have two main drawbacks: first, they usually cost a large amount of memory to store a scene due to the use of explicit data structures, such as voxels and octrees, which is not friendly enough for some low-end devices. Second, in the early training stage, these methods follow NeRF's framework of volume rendering, and dense sampling of the whole 3D space is unavoidable. This dense sampling to synthesis a pixel color hinder them from rendering a large patch of pixels during training for lacking enough GPU memory. Therefore, these methods are limited to using pixel-wise supervision and it is hard to adopt some image-level loss functions, e.g., perceptual loss~\cite{zhang2018perceptual} and CLIP loss~\cite{radford2021learning}, for a robust and semantic supervision.

% NeRF - Speed up without data structure
On the contrary, instead of using explicit data structures, some methods managed to build compact neural representations, while speed up the rendering of NeRF at the same time~\cite{piala2021terminerf,fang2021neusample,neff2021donerf} by predicting the surface distribution and reducing the point samplings. However, these neural representations for speed up heavily rely on either ground-truth depth maps~\cite{neff2021donerf} or the original NeRF densities~\cite{piala2021terminerf, fang2021neusample}. Therefore, at the training stage, if no ground truth depth values are provided, it is difficult to render a large patch of pixels at each iteration too.

% and some methods need heavy post processing from a pretrained NeRF~\cite{yu2021plenoctrees,reiser2021kilonerf,hedman2021baking}, and may lost information and reduce rendering quality. Very recently, DirectVoxGO~\cite{sun2021direct}, Plenoxels~\cite{yu2021plenoxels} and Instant-NGP~\cite{muller2022instant} reduce the training time of radiance fields by a very large degree, and even achieve real-time rendering. However, due to their either hybrid or non-neural representations, the memory consumption are still large.

\input{figures/fig_overfit}
% Light field
Another branch of works try to find a direct neural mapping from ray representations to colors, such mapping is also known as a neural {\it light field}. A {\it light field} is typically defined as a ray-color function, and usually with the assumption that the rendered color is constant with varing ray origins. This direct prediction has natural advantage to NeRF in terms of rendering speed, since it only needs single evaluation of the network to synthesis one pixel color. Besides, the single-evaluation property significantly decreases the GPU memory in each iteration of the training compared to that of NeRF. Therefore, neural light fields can render more pixels in each iteration, and are more suitable for image-level supervision.
However, compared to training a NeRF, it is much more difficult to train a neural light field. The main reason it that a neural radiance field, though a 5D function, is basically built on the 3D space, i.e., spatial positions~\cite{attal2021learning},
% and the spatial positions are early conditioned, and the extra two dimensions are actually lately conditioned~\cite{attal2021learning}.
which is naturally geometry-aware. On the contrary, to learn a neural light field, the network needs to find a direct mapping from rays to colors, where the ray is typically parameterized in the space of four or more dimensions. Also, this direct mapping contains nearly no information of the scene geometry, and naively training such network usually suffers from the problem of multi-view inconsistency~\cite{sitzmann2021light, attal2021learning}. That is, the network overfits the training images while can not generalize to novel views, as shown in Fig~\ref{fig:overfit}.


To deal with these issues, in this paper, we propose PCLFN for both a compact neural light field representation and an efficient rendering of forward-facing scenes. In the inference stage, PCLFN as the direct prediction method only queries the network once to synthesize a pixel color, which is more computationally efficient than NeRF. To address the problem of multi-view inconsistency of neural light field rendering, we propose a progressive training scheme. Specifically, in the early training stage, we de-active some neuron connects to the network, which, shown in the experiments, can provide a strong inductive bias for multi-view consistency. In this early stage, the architecture can also be seen as a set of tiny sub-networks. However, though geometry-aware and multi-view-consistent, the tiny sub-networks are not capable enough of encoding a complex scene. Therefore, we progressively increase the network capacity in the later training stage by adding more neuron connections. We note this progressive connection will weaken the multi-view consistency and propose a regularization scheme to help preserve the consistency. Once the training is done, we obtain a compact multi-layer perceptron (MLP) to represent the complex scene.

In summary, our contributions are:

\begin{itemize}
  \item A novel compact neural representation for encoding light fields and efficient view synthesis. This representation does not need any explicit data structures and is memory efficient (as small as 8MB) to store a complex scene.
  \item A progressive training scheme for the trading-off of the network capacity and multi-view consistency.
  \item A regularization scheme to help preserve multi-view consistency.
\end{itemize}



==> 3_method_bak.tex <==
\section{Method}
% Given a set of posed images as input, our goal is to render novel images give arbitrary poses as input. We assume that the images are captured in a similar camera rotation, therefore the view rays can be represented by two planes.

Given a set of forward-facing images with known camera poses, our goal is to learn a neural light field from these images. The inputs of our neural light field are the coordinates of rays and the outputs are corresponding rendered colors for these rays. In the following, we first introduce preliminaries about the two-plane 4D light field and the volume rendering.

\subsection{Preliminaries}
\input{figures/fig_preliminary}
{\bf Two-plane ray representation.} Since all cameras are forward-facing with similar directions, all rays in the scene can be represented by two points on the near plane and the far plane. As shown in Fig~\ref{fig:preliminary} (a), a ray is parameterized by $(u, v, s, t)$, where $(u, v)$ is the point coordinate of the near plane and $(s, t)$ is that of the far plane. Therefore, the light field, i.e., the ray-color mapping, can be modeled by a 4D function. Such function can be further encoded by a neural network $LF: \mathbb{R}^4\rightarrow \mathbb{R}^3$, where the input is the 4D coordinate and output is the corresponding RGB values.

% {\bf Multiple-plane images.} Given sparse image captures as supervision, directly encoding a 4D light field often suffers from multi-view inconsistency~\cite{sitzmann2021light,attal2021learning}. To obtain a geometry-consistent representation, one fashioned way is to model the scene as multiple plane images (MPI)~\cite{zhou2018stereo} as shown in Fig. xx. In this model, the 3D scene is represented by $D$ parallel RGB-A planes, where the last channel denotes the opacity of this position. Then the color for each ray can be rendered by alpha blending: 
% \vspace{2pt}

\noindent{\bf Volume rendering and MPI.} As shown in Fig~\ref{fig:overfit}, given sparse image captures as supervision, directly regressing a 4D light field with a neural network often suffers from multi-view inconsistency~\cite{sitzmann2021light,attal2021learning}, i.e., over-fitting to the training images and hard to generalize to novel views. One common way to obtain a multi-view consistent rendering results is introducing the 3D volume representation and using the volume rendering technique. With this technique, the 3D scene is typically represented by a color field, and a density field. Then to render a pixel color, one first samples a sequence of points $\{\mathbf{p}_0, ..., \mathbf{p}_{n-1}\}$ along the ray and query the corresponding sampled colors $\{c_0, ..., c_{n-1}\}$ as well as volume densities $\{\sigma_0, ..., \sigma_{n-1}\}$. The the color is synthesized by the volume accumulation as:

\begin{equation}
\begin{split}
    C &= \sum_{i=0}^{n-1} T_i{\alpha_i} c_i \\
    \alpha_i &= \delta_i\sigma_i \\
    T_i &= \prod_{j=0}^{i-1} (1 - \alpha_j).
    \label{eqn:volume_rendering}
\end{split}
\end{equation}

Here $\delta_i$ denotes the distance between $i$-th and $(i+1)$-th sampled point. Note that, another technique Multi-plane Image (MPI) for novel synthesis, shares a similar idea of volume rendering. With this technique, the 3D scene is represented by $D$ parallel planar RGB-$\alpha$ images, where the last channel stores the opacity information, similar to the concept of density. The planes are placed at the depths of $\{d_0, d_1, ..., d_{D-1}\}$ to a reference view frustum. To render a pixel color, we first find all intersections of the corresponding emitted ray with the planes and obtain the colors $\{c_0, c_1, ..., c_{D-1}\}$ and opacity $\{\alpha_0, \alpha_1, ..., \alpha_{D-1}\}$
%, which is similar to the sampling procedure in volume rendering.
Then the color is accumulated by Eqn~\ref{eqn:volume_rendering} similarly.

% We do not discuss the details of MPI, and refer the readers to Nex~\cite{wizadwongsa2021nex} for more information.

% Direct optimizing the multiple plane image would lead to noisy outputs, and is difficult to generalize to novel views~\cite{wizadwongsa2021nex}. Therefore, some methods tries to regularize the MPI by either direct predicting from CNN (cite). However, for CNN based methods, they only predict the view-independent RGBA values, therefore view-dependent effects, like specular colors, are difficult to model. The recent MPI method, Nex~\cite{wizadwongsa2021nex}, addressed this issue by indirect querying the RGBA information with a set of basis functions. However, in the training stage, since Nex encodes the MPI by coordinate-based networks, rendering the color of a ray needs hundreds of evaluations of the MLPs, which is time consuming and hard to perform image-level supervision.

% Next, we introduce PCLFN, to address the above issues.

\input{figures/fig_arch}
\subsection{Light Field Network Options}
As discussed already, direct training a function from light parameters to colors suffers over-fitting and multi-view inconsistency.
In this section, we introduce several possible alternatives of neural network architectures to both represent the light field and avoid multi-view inconsistency. The network architectures we discuss in this paper are all based on multi-layer perceptrons (MLPs).

% Without loss of generality, we assume the planes defined in the MPI are all parallel to the x-y plane in the world space. (Note that this space can be Euclidean space or NDC space..), and the planes are placed at z values of $\{d_1, d_2,...,d_D\}$, where $d_1=0$ and $d_D=1$.
\vspace{2pt}
\noindent{\bf Multiple-plane networks.} To synthesis the pixel color with multi-view consistency, one may follow the volume rendering technique, and define a set of multiple plane networks ({\bf MPNs} for abbreviation) $\{G_0, G_1, G_2,...,G_{D-1}\}$, where $G_i: \mathbb{R}^2 \rightarrow \mathbb{R}^4$ denotes the MLP encoding the color and opacity values of the i-th plane image, with the local x-y coordinates as input.

Without loss of generality, we assume the image planes are all parallel to the x-y plane in the world space, and the planes are placed at z values of $\{d_1, d_2,...,d_D\}$, where $d_1=0$ and $d_D=1$. Given a ray parameterized by the two-plane coordinates $(u, v, s, t)$, the color can be rendered using the volume accumulation by
\begin{equation}
\begin{split}
C(u, v, s, t) &= \sum T_i\alpha_i c_i \\
T_i &= \exp(-\sum{\alpha_i}) \\
\left[c_i | \alpha_i\right] &= G_i(x_i, y_i) \\
x_i &= u(1 - d_i) + s d_i \\
y_i &= v(1 - d_i) + t d_i.
\end{split}
\end{equation}

Since the RGB-$\alpha$ value of each sampled point is queried independently via the corresponding sub-network, MPNs can naturally ensure multi-view consistency. However, training such networks usually suffers from the trading-off of rendering quality and network complexity (as well as training difficulty). For example, to represent a scene in high fidelity, we usually need to use as many as 128 planes to build the multi-plane image. This means we need to train 128 sub-networks, which is very time-consuming for both training and inferring. An alternative is using a single network to globally represent all plane images, that is, given $(x_i, y_i, d_i)$ as input, the network output the corresponding color and opacity. This alternative representation is similar to NeRF~\cite{mildenhall2020nerf} and its variants. However, as shown in the past works~\cite{mildenhall2020nerf,liu2020neural,yu2021plenoctrees,reiser2021kilonerf,hedman2021baking} the rendering process is time-consuming too because it still needs hundreds of network evaluations to render the color for each ray.

\vspace{2pt}
\noindent{\bf Multiple-channel network.}
Another possible way is using a single network and directly predicting the RGB-$\alpha$ values of all the depth planes given a concatenation of x-y coordinates as input. Specifically, one may construct a multiple channel network ({\bf MCN} for short) $H: \mathbb{R}^{D\times 2} \rightarrow \mathbb{R}^{D\times 4}$; given the x-y coordinates $\{x_0,y_0,...x_{D-1},y_{D-1}\}$, the network directly outputs the RGB-$\alpha$ values of the intersections to the $D$ depth planes, and the pixel color is rendered in the same way in Eqn~\ref{eqn:volume_rendering}.

Since the sampled values are not independently conditioned on the spatial positions but queried in an entangled way, similar to direct color rendering as discussed in the introduction, naively optimizing MCN to fit the ground truth images also suffers from multi-view inconsistency. To improve the generalization ability to novel views, one may try to regularize the network by some loss designs.
% More details about the regularization can be found is Sec~\ref{sec:regularization}. 
However, as will be shown in the experiments, though somewhat helpful, using some regularization methods only would not achieve satisfactory results, especially when the images are sparse or the camera baselines are large.

We observe that the difficulty of regularization is mainly due to improper initialization. When the MCN is initialized with random weight parameters, it does not follow any multi-view consistency before training. Therefore it is challenging to regularize MCN in the training stage with only loss designs. On the contrary, we note that MPNs naturally have multi-view consistency since the sampled values are queried independently. The properties of MCN and MPNs motivate us to find a balance between the two network options.

\subsection{Progressively-connected Light Field Network}

In this section, we describe progressively-connected light field network (PCLFN), to provide a proper balance between MPNs and MCN. The key idea is that we first introduce a strong inductive bias to ensure multi-view consistency, with the help of MPNs, and then we progressively reduce the inductive bias while obtain larger network capacity, by adding more neuron connections. As will be shown the final form of PCLFN after training is similar to MCN.

% For the convenience of description, we make some conventions of the MLP's notation first. A multi-layer perceptron is typically recursively defined by

% \begin{equation}
% \begin{split}
%     z^i &= x\\
%     z^{i+1} &= \omega(W^{i}z^{i} + b^{i})\\
%     f(x) &= W^{k}z^{k} + b^{k}.
% \end{split}
% \label{eqn:mlp}
% \end{equation}
% Here $\omega$ is an activation function.

Specifically, we define the PCLFN at progress level $k$ with $D_k = D\times 2^{-k}$ sub-networks by $\Phi_{k} = \{F_k^0, F_k^1,...,F_k^{D_k-1}\}$, and each sub-network is with hidden width $W\times2^{k}$. Here $D$ and $W$ are preset parameters. For each $F_k^i: \mathbb{R}^{2\times 2^k} \rightarrow \mathbb{R}^{4\times 2^k}$, the input is a concatenation of the x-y coordinates $\{(x_j,y_j) | j = i\times 2^k, ..., (i+1)\times 2^k - 1\}$ from the corresponding depth planes, and the output is the corresponding concatenated RGB-$\alpha$ values. For each ray after querying all sub-networks, the color can be rendered by volume accumulation following Eqn.~\ref{eqn:volume_rendering}. It can be seen that the architecture of PCLFN is similar to MPNs when $k=0$ and to MCN when $k=\log_2(D)$.

We now describe how to train the network. The basic idea is that we divide the whole training into several stages and train PCLFN in a progressive manner. That is, we first optimize $\Phi1_0$ (MPNs), then in the following stages we gradually train $\Phi_1, \Phi_2, ...$ based on the lower level networks.
% We remark that along the training progress, the inductive-bias for multiview-consistency is gradually weakened, while the network capacity increases.

\vspace{2pt}
\noindent{\bf Progressive connection.}
Now we consider to increase the network capacity by merging the sub-networks at the end of each training stage. At the end of k-th training stage, we merge the sub-networks $F_k^{2i}$ and $F_k^{2i+1}$ to $F_{k+1}^{i}$ for $i \in [0, D\times 2^{-(k+1)})$. Formally, consider constructing the weight matrix $W_{k+1}^{i}$ and bias vector $b_{k+1}^i$ of each layer function $z_{k+1}^{i} = \omega(W_{k+1}^{i}y_{k+1}^{i} + b_{k+1}^i)$ of the MLP, where $y$ and $z$ are the input and output of the layer, and $\omega$ is either an activation function or identity function. Given the concatenation of the input $y_{k+1}^{i} = \left[y_k^{2i}, y_k^{2i+1}\right]$, we expect the output is also the corresponding concatenation, i.e., $z_{k+1}^{i} = \left[z_k^{2i}, z_k^{2i+1}\right]$. To this end, we construct the weight matrix and bias vector as
\begin{equation}
    W_{k+1}^{i} = \begin{bmatrix} W_{k}^{2i} & 0 \\ 0 & w_{k}^{2i+1} \end{bmatrix}, b_{k+1}^{i} = \left[ b_{k}^{2i}, b_{k}^{2i+1} \right].
\end{equation}


\vspace{2pt}
\noindent{\bf Subdivide output depth planes.} Besides increasing network capacity by adding more neuron connections, we can further improve the rendering quality by subdivide the output depth planes. Specifically, consider the last linear layer of the network as function $z = Wy + b$, we construct the new weight matrix and bias vector $\hat{W}, \hat{b}$ by self copy of $W$ and $b$ (a little hard to explain...)

\subsection{Regularization}
\label{sec:regularization}
Note that such neuron connection will destroy the constraints for multi-view consistency and as the training proceeds the network may overfit the training views. Therefore, we need to further regularize the network by adding extra losses design.

\input{figures/fig_epi}
\vspace{2pt} 
\noindent{\bf Sampled consistency loss.} The progressive connection of neurons makes the queried value of each depth sample entangled with other samples. Therefore we propose a loss to ease the entanglement issue to keep multiview consistency. For convenience of description, we define a proxy function $L(u, v, s, t) = \Phi(\gamma(u, v, s, t))_{i,j}$, where $\sigma$ is the mapping function to the concatenation of the sampled x-y coordinates at depth planes $\{d_0, d_1, ... d_{D-1}\}$, $\Phi$ is the light field network. Note that in this context we assume the output of $\Phi$ is a $D\time 4$ matrix denoting the sampled RGB-$\alpha$ values. Ideally, the value of $L$ should be independently queried by the local coordinate $(x_i, y_i)$, where $x_i = u(1-d_i) + sd_i$, $y_i = v(1 - d_i) + td_i$. That is, for the fixed 3D point at depth plane $d_i$, with 3D coordinate $(x_i, y_i, d_i)$, $(u', v', s', t')=(u, v, s, t) + (d_i p, d_i q, (1-d_i) p, (1-d_i) q)$, there is $x'_i=x_i, y'_i = y_i$, where $p, q$ are the arbitrary values, $(x'_i, y'_i)$ is the local x-y coordinate of the intersection between ray $(u', v', s', t')$ and the depth plane $d_i$. The value of $L(u, v, s, t)$ and $L(u', v', s', t')$ is expected the same. Therefore we propose a consistency loss that
\begin{equation}
\begin{split}
    \mathcal{L}_{\rm sample} &= \|\nabla L(u, v, s, t)\cdot \mathbf{p})\|^2 + \|\nabla L(u, v, s, t)\cdot \mathbf{q}) \|^2 \\
    \mathbf{p} &= (d_i, 0, (1 - d_i), 0)^{\top} \\
    \mathbf{q} &= (0, d_i, 0, (1 - d_i))^{\top}.
\end{split}
\end{equation}
Note that we need to compute all the loss term for every queried value (color or opacity) with difference depth planes. In practice, we first compute the Jacobian matrix of $\Phi$ then compute all the sampled consistency loss terms.

\vspace{2pt} 
\noindent{\bf Accumulated consistency loss.} In our early experiment we found that supervising the gradient of each samplings individually would not achieve satisfied result, showing some image flickings when camera moves. We think the problem is due to the accumulation error from the volume rendering equation. That is, though the consistency errors of each sampled values are small, the accumulated color by volume rendering may still suffer multi-view inconsistency. To this end, we propose accumulated consistency loss for regularized the rendered colors. For the ray $(u, v, s, t)$ and the rendered color $C(u, v, s, t)$, if the depth $\hat{d}$ of the intersected surface is known, then similar to the sampled consistency loss, for the neighboring rays $(u', v', s', t')=(u, v, s, t) + (\hat{d} p, \hat{d} q, (1-\hat{d}) p, (1-\hat{d}) q)$, the rendered color should be the same. Therefore we propose the loss by
\begin{equation}
\begin{split}
    \mathcal{L}_{\rm accum} &= \mathcal{R}(\nabla C(u, v, s, t)\cdot \mathbf{p}) + \mathcal{R}(\nabla C(u, v, s, t)\cdot \mathbf{q}) \\
    \mathbf{p} &= (\hat{d}, 0, (1 - \hat{d}), 0)^{\top} \\
    \mathbf{q} &= (0, \hat{d}, 0, (1 - \hat{d}))^{\top} \\
    \hat{d} &= \sum_{i} T_i\alpha_i d_i.
\end{split}
\end{equation}

Here $T_i$ and $\alpha_i$ follows the same definition as Eqn.~\ref{eqn:volume_rendering}, and $\mathcal{R}$ is chosen as smooth L1 loss~\cite{girshick2015fast} for less sensitivity to out-liers on occlusion boundaries. The intuition of this loss can be shown in Fig~\ref{fig:epi}.


\input{figures/fig_depth}


==> figures/fig_depth.tex <==
\begin{figure}[htb]
  \includegraphics[width=\linewidth]{figure_resources/depth.pdf}
  \caption{}
  \label{fig:depth}
\end{figure}

==> figures/fig_epi.tex <==
\begin{figure}[htb]
  \includegraphics[width=\linewidth]{figure_resources/epi.pdf}
  \caption{}
  \label{fig:epi}
\end{figure}

==> supp_tables/flops.tex <==
\begin{table}[htb]
    \begin{tabular}{c|c|c|c|c|c|c}
        \hline
        & ProLiF$_0$ & ProLiF$_1$ & ProLiF$_2$ & ProLiF$_3$ & ProLiF$_4$ & NeRF \\
        \hline
        FLOPs & 0.13M & 0.27M & 0.57M & 1.25M & 2.88M & 109M
    \end{tabular}
    \caption{{\bf FLOPs comparison.} }
    \label{tab:supp_flops}
\end{table}


==> tables/model_size_flops.tex <==
\begin{table}
    \begin{tabular}{c||c|c|c|c||c}
       & PCLFN & NeRF & PCLFN & dw\\
       \hline
      Direct training
      & 16.89 & 25.03 & 22.84 & 22.47 & 21.81 \\
      w/o Reg. 
      & 16.37 & 25.11 & 22.41 & 22.73 & 21.65 \\
      w/o Prog.
      & 19.33 & 29.56 & 25.35 & 25.37 & 24.91 \\
      Full Model
      & 19.94 & 30.23 & 25.84 & 26.86 & 25.72 \\
    \end{tabular}
    \label{tab:model_size_flops}
\end{table}
